Hand-Object Interaction Controller (HOIC): Deep Reinforcement Learning for Reconstructing Interactions with Physics

Hand manipulating objects is an important interaction motion in our daily activities. We faithfully reconstruct this motion with a single RGBD camera by a novel deep reinforcement learning method to leverage physics. Firstly, we propose object compensation control which establishes direct object control to make the network training more stable. Meanwhile, by leveraging the compensation force and torque, we seamlessly upgrade the simple point contact model to a more physical-plausible surface contact model, further improving the reconstruction accuracy and physical correctness. Experiments indicate that without involving any heuristic physical rules, this work still successfully involves physics in the reconstruction of hand-object interactions which are complex motions hard to imitate with deep reinforcement learning. Our code and data are available at https://github.com/hu-hy17/HOIC.

==> sections/preliminary.tex <==
\section{Preliminary}
%
In this section, we will briefly introduce the fundamentals of reinforcement learning \cite{sutton1998introduction}, which serve as the foundation of our method.
%
Reinforcement learning aims to find an optimal solution for a sequential decision process.
%
In the process, an agent interacts with the environment according to a policy $\pi$ which is typically represented as a conditional distribution.
%
At each time step of the sequence, the agent observes the state $s_t$ of the environment and takes an action $a_t$ sampled from the distribution $\pi(a|s)$.
%
After taking the action, the agent receives a reward $r(s_t, a_t)$ and the new state $s_{t+ 1}$.
%
The optimization objective is to find the optimal distribution $\pi(a|s)$ that maximizes the accumulated rewards over the entire sequence, written as:

\begin{equation}\label{eq:totalrwd}
   \arg\max\limits_{\pi} E_{\tau \sim p_{\pi}(\tau)}\left(\sum_{t}r(s_t, a_t)\right),
\end{equation}
where $\tau$ is the whole sequence $[s_0, a_0, s_1, a_1, ..., s_T, a_T]$ and $p_{\pi}(\tau)$ is the distribution of $\tau$ when the agent follows the policy $\pi$.
%

\HHY{This paragraph is not necessary}Deep reinforcement learning (DRL) uses a neural network to represent the policy, enabling the learning of complex mappings between high-dimensional environmental states and actions. 
%
To train the policy network, a widely used algorithm is policy gradient, where the derivative of the optimization objective with respect to the network parameters is calculated as:

%\begin{equation}\label{eq:pg}
%\nabla_{\theta} J(\theta) \approx \frac{1}{N}\sum_{i=1}^{N}\left(\sum_{t=1}^T \nabla_{\theta}\log\pi_{\theta}(a_{i,t}|s_{i,t})\right)\left(\sum_{t=1}^T r(s_{i,t}, a_{i,t})\right)
%\end{equation}

\begin{equation}\label{eq:pg}
\nabla_{\theta} J(\theta) = E_{\tau \sim p_{\pi_\theta}(\tau)}\left(\sum_{t=1}^T \nabla_{\theta}\log\pi_{\theta}(a_{t}|s_{t})\right)\left(\sum_{t=1}^T r(s_{t}, a_{t})\right),
\end{equation}
where $J(\theta)$ is the optimization objective mentioned above, $\pi_\theta$ is the policy represented using network with parameter $\theta$.
%
In practice, the expectation in Eq.~\ref{eq:pg} is approximated by sampling a collection of trajectories with policy $\pi_\theta$. 


